AMB3R: Accurate Feed-forward Metric-scale 3D Reconstruction with Backend

We present AMB3R, a multi-view feed-forward model for dense 3D reconstruction on a metric-scale that addresses diverse 3D vision tasks. The key idea is to leverage a sparse, yet compact, volumetric scene representation as our backend, enabling geometric reasoning with spatial compactness. Although trained solely for multi-view reconstruction, we demonstrate that AMB3R can be seamlessly extended to uncalibrated visual odometry (online) or large-scale structure from motion without the need for task-specific fine-tuning or test-time optimization. Compared to prior pointmap-based models, our approach achieves state-of-the-art performance in camera pose, depth, and metric-scale estimation, 3D reconstruction, and even surpasses optimization-based SLAM and SfM methods with dense reconstruction priors on common benchmarks.

==> tab/3d.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
    \begin{tabularx}{\textwidth}{r *{12}{>{\centering\arraybackslash}X}}
      \toprule

      \multirow{3}{*}{Method} & \multicolumn{4}{c}{7 scenes} & \multicolumn{4}{c}{NRGBD} & \multicolumn{4}{c}{Eth3D} \\

      \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
        & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} \\
      \midrule
      \textbf{Dust3R$^\dagger$}
        & \bf 0.0286 & \bf 0.0123 & 0.0280 & 0.0091 & \bf 0.0544  & \bf 0.0251  & 0.0315  & \bf 0.0103 & - & - & - & - \\
      \textbf{Spann3R}
        & 0.0342 & 0.0148 & \bf 0.0241 & \bf 0.0085 & 0.0691  & 0.0315  & \bf 0.0291  & 0.0110 & - & - & - & - \\

      \textbf{VGGT}
        & 0.0342 & 0.0148 & \bf 0.0241 & \bf 0.0085 & 0.0691  & 0.0315  & \bf 0.0291  & 0.0110 & - & - & - & - \\

       \textbf{Ours}
        & 0.0137 & 0.004 & \bf 0.0236 & \bf 0.0103 & 0.0691  & 0.0315  & \bf 0.0291  & 0.0110 & - & - & - & - \\
      \bottomrule
    \end{tabularx}%
    \vspace{-5pt}
    \caption{\textbf{Quantitative results on 7Scenes, NRGBD, and ETH3D datasets.} DUSt3R$^\dagger$ indicates using DUSt3R's final weights on $224\times 224$ images, same as our input resolution, to fit within 24GB GPU memory. For few-view (FV) reconstruction, we use the 8-frame pairs as in SimpleRecon. Note that evaluating DUSt3R at the original resolution may benefit from increased visual overlap.}
    \label{tab:quantitative_modified}
\end{table*}

==> tab/ablation_metric.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|}

\hline
    \textbf{Method}
    & \multicolumn{2}{c|}{\textbf{\kittishort{}}}
    & \multicolumn{2}{c|}{\textbf{\scannetshort{}}}
    & \multicolumn{2}{c|}{\textbf{\ethdshort{}}}
    & \multicolumn{2}{c|}{\textbf{\dtushort{}}}
    & \multicolumn{2}{c|}{\textbf{\tanksandtemplesshort{}}}
    \\

    & $\absrel\!\downarrow$ & $\delta_{1.25}\!\uparrow$
    & $\absrel\!\downarrow$ & $\delta_{1.25}\!\uparrow$
    & $\absrel\!\downarrow$ & $\delta_{1.25}\!\uparrow$
    & $\absrel\!\downarrow$ & $\delta_{1.25}\!\uparrow$
    & $\absrel\!\downarrow$ & $\delta_{1.25}\!\uparrow$
    \\
    \hline


\hline
\end{tabular}}
\caption{Ablation study on metric-scale prediction.}
\end{table}
